Graphs and colorings for answer set programming

We investigate the usage of rule dependency graphs and their colorings for characterizing and computing answer sets of logic programs. This approach provides us with insights into the interplay between rules when inducing answer sets. We start with different characterizations of answer sets in terms of totally colored dependency graphs that differ in graph-theoretical aspects. We then develop a series of operational characterizations of answer sets in terms of operators on partial colorings. In analogy to the notion of a derivation in proof theory, our operational characterizations are expressed as (non-deterministically formed) sequences of colorings, turning an uncolored graph into a totally colored one. In this way, we obtain an operational framework in which different combinations of operators result in different formal properties. Among others, we identify the basic strategy employed by the noMoRe system and justify its algorithmic approach. Furthermore, we distinguish operations corresponding to Fitting's operator as well as to well-founded semantics. (To appear in Theory and Practice of Logic Programming (TPLP))

==> Proofs/LongVersion/cor_PU_empty_exists.tex <==
\begin{proof}{cor:PUast:empty:exists}
Proof by induction by Theorem~\ref{thm:inductive:propPU}.
\end{proof}

==> Proofs/LongVersion/cor_max_supported_graph_existence.tex <==
\begin{proof}{cor:max:supported:graph:existence}
\comment{K2T:please, check}
  Let $\bg{}$ be the \RDGraph{} of logic program $\Pi$
  and
  $\col$ be a partial coloring of \bg{}.

Furthermore, let $X\in \AS{\Pi}{\col}$ be an answer set such that $\colplus
\subseteq 
\GR{\Pi}{X}$ and $\colminus \cap \GR{\Pi}{X}=\emptyset$.

We want to construct a support graph $(\GR{\Pi}{X},E)$ of $(\bg{},C)$ for some
$Esubseteq (\Pi\times\Pi)$.
Then, we know that there exists a maximal support graph of $(\bg{},C)$.
\comment{K2TS: does this step work?}

By Theorem~\ref{thm:gr:grounded} we have an enumeration  $\langle r_i
\rangle_{i \in I}$ of \GR{\Pi}{X} such 
that for all $i \in I$ we have $\pbody{r_i} \subseteq \head{\{r_j \mid j <
  i\}}$. 

Let $V^0=\{r_0\}$ and $E^0=\emptyset$.
Assume, $V^i$ and $E^i$ are constructed for some $i < \omega$.
Define
\(
V^{i+1}=V^i\cup\{r_i\}
\)
and
\(
E^{i+1}=E^i\cup E^{r_i}
\)
where
\[
E^{r}=\bigcup_{p\in \pbody{r}} \{(\rp,\r) \mid \rp\in V^i, \head{\rp}=p\}.
\]
Then, $(V,E)= \left( \bigcup_{i < \omega} V^i, \bigcup_{i< \omega} E^i
\right)$.
Clearly, $V=\GR{\Pi}{X}$ by construction and thus, $\colplus \subseteq V$ and
$\colminus \cap V =\emptyset$.
Furthermore, $(V,E)$ is a support graph of $\bg{}$ by
Definition~\ref{def:acol:Dasg} and by construction of $V$ and $E$.

% We have $\colplus \subseteq \GR{\Pi}{X}$. Then, from
% Theorem~\ref{thm:gr:grounded} we have that there exists an enumeration
% $\langle r_i \rangle_{i\in I}$ of $\GR{\Pi}{X}$ such that
% $\pbody{r_i}\subseteq \head{\{r_j\mid j<i\}}$.
% Hence, we have an enumeration $\langle r_i \rangle_{i\in J}$ of $\colplus$. 

% Starting from this enumeration we want to construct the support graph
% $(\colplus,E)$ of $\bg{}|_\col$. 
% Let $(V^0,E^0)=(\emptyset,\emptyset)$ and $(V^1,E^1)=(\{r_1\},\emptyset)$.
% Clearly, we must have $\pbody{r_1}=\emptyset$.
% For this reason we can define $E^1=\emptyset$.
% Assume, that we have constructed $(V^i,E^i)$ for some $i < |J|$.
% Then, $(V^{i+1},E^{i+1})=(V^i\cup \{r_{i+1}\},E^i\cup E^{r_{i+1}})$ where
% $E^{r_{i+1}}= \bigcup_{p\in \pbody{r_{i+1}}} \{(\rp,r_{i+1})\mid \rp\in V^i,
% \head{\rp}=p, (\rp,r_{i+1})\in \bgezero\}$.

% For $n=|J|$ we have that $(V^n,E^n)=(\colplus,E')$ is a support graph of
% $\bg{}|_\col$. 

\end{proof}
%%% Local Variables: 
%%% mode: latex
%%% TeX-master: t
%%% End: 


==> Proofs/LongVersion/cor_nlp_properties.tex <==
\begin{proof}{cor:nlp:properties}
Let $\bg{}$ be the \RDGraph\ of logic program $\Pi$,
$\col$ be a total
coloring 
of $\bg{}$ and $\{X\} = \AS{\Pi}{\col}$.
By definition of $X$ we have $\colplus = \GR{\Pi}{X}$ and 
$\head{\colplus} = X$ (by Theorem~\ref{thm:X:headcolplus}).  
%
Since $\col$ is a total coloring we only have to show the ``$\Rightarrow$''
direction, because "$\Leftarrow$" is fulfilled through
Theorem~\ref{thm:nlp:properties}. 
%

\paragraph{Show condition 1 "$\Rightarrow$":}
% 
Let $\pbody{\r}\subseteq X=\head{\colplus}$ for $\r \in \Pi$.
%
Then, for each $p \in \pbody{\r}$ there exists an $\rp \in \Pi$ such that
$\rp\in\colplus$ and $p=\head{\rp}$.
%
From the definition of the \RDGraph\ we can conclude that $\r \in
S(\bg{},\col)$. 
%
\paragraph{Show condition 2 "$\Rightarrow$":}
%
Let $\r\in\Pi$ be such that $p \not\in X=\head{\colplus}$ for some $p \in
\pbody{\r}$. 
%
Then, for all \rp\ such that  $\head{\rp}=p $ we have $\rp\in\colminus$ and
it follows that $\r\in \overline{S}(\bg{},\col)$.
%
\paragraph{Show condition 3 "$\Rightarrow$":}
% 
There exists a $p \in \nbody{\r}$ such that $p \in X=\head{\colplus}$.
% 
Therefore, there exists an $\rp \in \GR{\Pi}{X}=\colplus$ such that
$\head{\rp}=p$ and $\rp\in\colplus$.
%
From the definition of the \RDGraph\ follows that $\r\in B(\bg{},\col)$.  
%
 \paragraph{Show condition 4 "$\Rightarrow$":}
% 
For all $q \in \nbody{\r}$ we have $q \not\in X$.
% 
From the definition of $X=\head{\colplus}$  for all $\rp  \in \Pi$ with
$\head{\rp}= q$ we have
that $\rp\in\colminus$.
% 
From the definition of the \RDGraph\ we can conclude that  $\r \in
\overline{B}(\bg{},\col)$.  
%


\end{proof}
%----------------------------------------------------------------
%% Local Variables: 
%%% mode: latex
%% TeX-master: "~/tex/Papers/GraphLP/Grundlagen/paper"
%%% End: 


==> Proofs/LongVersion/prop_extension_defined.tex <==
\begin{proof}{prop:extension:defined}
   Let $\bg{}$ be the \RDGraph{} of logic program $\Pi$
   and \col{} a partial coloring of \bg{}.

We have to show that $\fOPprop{\bg{}}{\col}$ is a partial coloring.
But this holds since 
\[(S (\bg{},\col) \cap \overline{B}(\bg{},\col)) \cap
(\overline{S}(\bg{},\col) \cup B (\bg{},\col)) =\emptyset
\]
by Definition~\ref{def:acol:vertexproperties}. 

\end{proof}
%%% Local Variables: 
%%% mode: latex
%%% TeX-master: t
%%% End: 


==> Proofs/LongVersion/thm_P_monoton.tex <==
\begin{proof}{thm:P:monoton}
  Let \bg{} be the \RDGraph{} of logic program $\Pi$ 
  and
  let $\col$ and $\col'$ be partial colorings of \bg{} such that
  $\AC{\Pi}{\col'}\neq\emptyset$.
Then $\AS{\Pi}{C'}\not=\emptyset$ by
  Theorem~\ref{thm:AS:AC}.
Furthermore, let be $\col\sqsubseteq\col'$.
Then, we also have $\AS{\Pi}{C}\not=\emptyset$ by definition.

\paragraph{$\fOPprop{\bg{}}{\col}\sqsubseteq\fOPprop{\bg{}}{\col'}$:}
It is easy to see that $\col \sqsubseteq \col'$ implies
\begin{enumerate}
\item $S(\bg{},\col) \subseteq S(\bg{},\col')$,
\item $\overline{S}(\bg{},\col) \subseteq \overline{S}(\bg{},\col')$,
\item $B(\bg{},\col) \subseteq B(\bg{},\col')$ and
\item $\overline{B}(\bg{},\col) \subseteq \overline{B}(\bg{},\col')$.
\end{enumerate}
Thus, $\fOPprop{\bg{}}{\col}\sqsubseteq\fOPprop{\bg{}}{\col'}$.

\paragraph{$\fOPpropast{\bg{}}{\col}\sqsubseteq\fOPpropast{\bg{}}{\col'}$:} 
By Theorem~\ref{thm:inductive:prop} property~7 it is enough to show
that 
$P(C)\sqsubseteq P(\col')$. 
Thus, it remains to show, that $P^i(C) \sqsubseteq P^i(C')$ for all $i <
\omega$. 
We prove this by induction over $i$.
For $i=0$ we have $P^0(C)=C \sqsubseteq C' = P^0(C')$.
Assume that $P^i(C) \sqsubseteq P^i(C')$ for some $ i < \omega$.
We have to show that $P^{i+1}(C) \sqsubseteq P^{i+1}(C')$.
But $P^{i+1}(C)=\fOPprop{\bg{}}{P^i(C)}\sqsubseteq
\fOPprop{\bg{}}{P^i(C')}=P^{i+1}(C')$ holds by the first half of this theorem.
% Also, it is easy to see that for $P^i(C) \sqsubseteq P^i(C')$ we have 
% \begin{enumerate}
% \item $S(\bg{},P^i(C)) \subseteq S(\bg{},P^i(C'))$,
% \item $\overline{S}(\bg{},P^i(C)) \subseteq \overline{S}(\bg{},P^i(C'))$,
% \item $B(\bg{},P^i(C)) \subseteq B(\bg{},P^i(C'))$ and
% \item $\overline{B}(\bg{},P^i(C)) \subseteq \overline{B}(\bg{},P^i(C'))$.
% \end{enumerate}
% Thus, $P^{i+1}(C) \sqsubseteq P^{i+1}(C')$.

\end{proof}
%%% Local Variables: 
%%% mode: latex
%%% TeX-master: t
%%% End: 


==> Proofs/LongVersion/thm_U_unsupported.tex <==
\begin{proof}{thm:U:unsupported}
\comment{K2T: weiß gar nicht, ob wir das noch brauchen}
Let $\bg{}$ be the \RDGraph\ of logic program $\Pi$ and $\col$ be a partial
coloring of $\bg{}$.
Furthermore let $X\in \AS{\Pi}{\col}$ be an answer set such that
$\colplus=\GR{\Pi}{X}$, $\head{\colplus}=X$ and $\colminus=\emptyset$.

By Theorem~\ref{thm:max:supported:graph:existence} there exists a maximal
support graph $(V,E)$ of $(\bg{},\col)$ for some $E\subseteq (\Pi\times\Pi)$.
Thus, $\fOPMaxGround{\bg{}}{\col}=(\colplus,\colminus\cup(\Pi\setminus V))$ by
definition of $\OPMaxGround_{\bg{}}$.
By $\colminus=\emptyset$ we have
$\fOPMaxGround{\bg{}}{\col}=(\colplus,(\Pi\setminus V))$.
We have to show that $\Pi\setminus V=\{\r\mid \pbody{\r}\not\subseteq X\}$.
\paragraph{Show "$\subseteq$":}
Assume that there exists an $\r\in \Pi\setminus V$ such that
$\pbody{\r}\subseteq X$.
Then, $\pbody{\r}\subseteq  \head{\colplus}$ and we have \r\ is supported in
$(\bg{},\col)$ by definition of supported and the \RDGraph.
By the maximality of $V$ we have then $\r\in V$.
But that's a contradiction.
Thus, for all $\r\in \Pi\setminus V$ we have $\pbody{\r}\not\subseteq X$.
\paragraph{Show "$\supseteq$":}
Let $\r\in \Pi$ such that $\pbody{\r}\not\supseteq X=\head{\colplus}$.
We have to show that $\r\in \Pi\setminus V$.
But that is obvious because \r\ can not be in $V$ because \r\ is not
supported in $(\bg{},\col)$ by definition of supportness.

\end{proof}
%%% Local Variables: 
%%% mode: latex
%%% TeX-master: t
%%% End: 


==> Proofs/LongVersion/thm_col_gr.tex <==
\begin{proof}{thm:col:gr}
  Let $\bg{}$ be the \RDGraph{} of logic program  $\Pi$,
  $\col$ be a partial coloring of $\bg{}$ and 
  $X \in \AS{\Pi}{\col}$ be an answer set.

\paragraph{Show 1:}
We have to show that for $\r\in S(\bg{},\col)\cap\overline{B}(\bg{},\col)$ we
have $\r \in \GR{\Pi}{X}$.
%
By Theorem~\ref{thm:nlp:properties} we have
$\pbody{\r}\subseteq X$ and $\nbody{\r} \cap X=\emptyset$.
%
Thus, $\r\in \GR{\Pi}{X}$.
\paragraph{Show 2:}
We have to show that for $\r\in
\overline{S}(\bg{},\col)\cup B(\bg{},\col)$ we 
have $\r \not\in \GR{\Pi}{X}$.
%
From Theorem~\ref{thm:nlp:properties} we can conclude that $\pbody{\r}
\not\subseteq X$ or $\nbody{\r}\cap X \not=\emptyset$ .
%
Thus, $\r \not\in \GR{\Pi}{X}$.

Analogously, we have condition~3 and~4 by
Corollary~\ref{cor:nlp:properties}.  
\end{proof}

%%% Local Variables: 
%%% mode: latex
%%% TeX-master: t
%%% End: 


==> Proofs/LongVersion/thm_inductive_propT_T.tex <==
\begin{proof}{thm:inductive:propT:T}
  Let \bg{} be the \RDGraph{} of logic program $\Pi$ and \col{} a partial
  coloring of \bg{}.

\paragraph{"$\sqsupseteq$":}
We have to show:
\begin{enumerate}
\item $T(C)$ is a partial coloring,
\item $\col \sqsubseteq T(C)$,
\item $T(C)$ is closed under $\mathcal{T}_{\bg{}}$.
\end{enumerate}
By Theorem~\ref{thm:inductive:propT} we have $T(C)$ is a partial coloring and
$\col \sqsubseteq T(C)$ by definition of $T(C)$.
Thus, it remains to show, that $T(C)$ is closed under $\mathcal{T}_{\bg{}}$.
\tbf

\paragraph{"$\sqsubseteq$":}
We prove this by induction over $i$.
For $i=0$ we have $T^0(C)=C \sqsubseteq \weakProp{\bg{}}{\col}$ by definition
of $\mathcal{T}^\ast_{\bg{}}$.
Assume that $T^i(C) \sqsubseteq \weakProp{\bg{}}{\col}$ for some $i < \omega$.
We have to show that $T^{i+1}(C) \sqsubseteq \weakProp{\bg{}}{\col}$.
By definition we have
$T^{i+1}(C)  = T^i(C) \sqcup \mathcal{T}_{\bg{}}(T^i(C))$.
By $T^i(C) \sqsubseteq \weakProp{\bg{}}{\col}$ and $\mathcal{T}^\ast_{\bg{}}$ is
closed under $\mathcal{T}_{\bg{}}$ we have $T^{i+1}(C) \sqsubseteq
\weakProp{\bg{}}{\col}$. 
\end{proof}
%%% Local Variables: 
%%% mode: latex
%%% TeX-master: "~/tex/Papers/Preference/Acolorings/paper"
%%% End: 


==> Proofs/LongVersion/thm_inductive_prop_P.tex <==
\begin{proof}{thm:inductive:prop:P}
\comment{ok}

This theorem follows directly from Theorem~\ref{thm:inductive:prop} and from
the definition of $\OPpropast{\bg{}}$.

%   Let \bg{} be the \RDGraph{} of logic program $\Pi$, \col{} a partial
%   coloring of \bg{} and $\AS{\Pi}{\col}\neq\emptyset$.

% \paragraph{"$\sqsupseteq$":}
% We have to show:
% \begin{enumerate}
% \item $P(\col)$ is a partial coloring,
% \item $\col \sqsubseteq P(\col)$,
% \item $P(\col)$ is closed under $\OPprop{\bg{}}$.
% \end{enumerate}
% By Theorem~\ref{thm:inductive:prop} we have that $P(\col)$ is a partial coloring
% and by $\col=P^0(\col)$ we have $\col \sqsubseteq P(\col)$.
% Thus, it remains to show, that $P(\col)$ is closed under $\OPprop{\bg{}}$.
% \tbf

% \paragraph{"$\sqsubseteq$":}
% We prove this by induction over $i$.

% For $i=0$ we have $P^0(\col)=\col \sqsubseteq \fOPpropast{\bg{}}{\col}$
% by definition of $\OPpropast{\bg{}}$.
% We assume that $P^i(\col) \sqsubseteq \fOPpropast{\bg{}}{\col}$ for some $i <
% \omega$.
% We have to show that $P^{i+1}(\col) \sqsubseteq \fOPpropast{\bg{}}{\col}$.
% We have $P^{i+1}(\col)=\fOPprop{\bg{}}{P^i(\col)} \sqcup
% P^i(\col)$.
% By $P^i(\col) \sqsubseteq \fOPpropast{\bg{}}{\col}$ and $\OPpropast{\bg{}}$ is
% closed under $\OPprop{\bg{}}$ we get $P^{i+1}(\col) \sqsubseteq
% \fOPpropast{\bg{}}{\col}$. 


\end{proof}
%%% Local Variables: 
%%% mode: latex
%%% TeX-master: "~/tex/Papers/GraphLP/Grundlagen/paper"
%%% End: 


==> Proofs/LongVersion/thm_max_supported_graph_existence.tex <==
\begin{proof}{thm:max:supported:graph:existence}
  Let $\bg{}=(\Pi,\bgezero,\bgeone)$ be the \RDGraph{} of logic program $\Pi$
  and
  $\col$ be a partial coloring of \bg{}.

We abbriviate $\bg{}|_{\colplus\cup \colminus}$ with $\bg{}|_C$.
%% We have to prove
%%   \begin{enumerate}
%%   \item   If $\AC{\Pi}{\col}\not=\emptyset$,
%%   then there is a (maximal) \groundedZeroDAG\ of $(\bg{},\col)$.
%%   \item If $(\colplus,E)$ is a \groundedZeroDAG\ of $\bg{}|_\col$
%%   for some $E \subseteq (\Pi\times \Pi)$,
%%   then there is a (maximal) \groundedZeroDAG\ of $(\bg{},\col)$.
%%   \end{enumerate}


\paragraph{Show~1:}
If $\AC{\Pi}{\col}\not=\emptyset$ then $\AS{\Pi}{\col}\not=\emptyset$ by
Theorem~\ref{thm:AS:AC}. 
Let $X\in \AS{\Pi}{C}$. Then by definition $\colplus\subseteq \GR{\Pi}{X}$ and
$\colminus 
\cap \GR{\Pi}{X}=\emptyset$.
We want to construct a support graph $(\GR{\Pi}{X},E)$ of $(\bg{},C)$ for some
$E\subseteq (\Pi\times\Pi)$.
Also, there exists then a maximal support graph of $(\bg{},C)$.

By Theorem~\ref{thm:gr:grounded} we have an enumeration  $\langle r_i
\rangle_{i \in I}$ of \GR{\Pi}{X} such 
that for all $i \in I$ we have $\pbody{r_i} \subseteq \head{\{r_j \mid j <
  i\}}$. 

%% Let $V^0=\{r_0\}$ and $E^0=\emptyset$.
%% Assume, $V^i\subseteq \Pi$ and $E^i\subseteq \Pi\times\Pi$ are constructed for
%% some $i < \omega$. 
%% Define
%% \(
%% V^{i+1}=V^i\cup\{r_i\}
%% \)
%% and
%% \(
%% E^{i+1}=E^i\cup E^{r_i}
%% \)
%% where
%% \[
%% E^{r_i}=\bigcup_{p\in \pbody{r_i}} \{(\rp,\r_i) \mid \rp\in V^i, \head{\rp}=p\}.
%% \]
%% Then, $(V,E)= \left( \bigcup_{i < \omega} V^i, \bigcup_{i< \omega} E^i
%% \right)$.
Define $V=\bigcup_{i\in I} \{r_i\}$ and
\(
E=\{(r_j,r_i)\mid j < i\}\cap \bgezero
\).
Clearly, $V=\GR{\Pi}{X}$ by construction and thus, $\colplus \subseteq V$,
$\colminus \cap V =\emptyset$, and $(V,E)$ is a support graph of $\bg{}$.
Thus, $(V,E)$ is a support graph of $(\bg{},C)$ by construction of $V$.
The existence of a maximlaity one follows by Theorem~\ref{prop:SG:existence}.

\paragraph{Show~2:}
Let $(\colplus,E')$ be a support graph of $\bg{}|_\col$ for some
$E' \subseteq (\Pi \times \Pi)$.
%% With Definition~\ref{def:acol:maxgrounded} we have to show, that there exists
%% a (maximal) support graph $(V,E)$ of $\bg{}$ such that $\colplus \subseteq V$ and
%% $\colminus \cap V=\emptyset$.

Now, we want to extend $(\colplus,E')$ to a support graph $(V,E)$ of $\bg{}$
such that $\colplus \subseteq V$ and $\colminus \cap V=\emptyset$.
Let 
\[(V^0,E^0)=(\colplus,E').\]
Assume, that we have constructed $(V^i,E^i)$ for $0 < i < \omega$.
We define, 
\[(V^{i+1},E^{i+1})=(V^i \cup \{r_{i+1}\},E^i\cup E^{r_{i+1}})\]
 where 
$\r_{i+1} \in \Pi \setminus (V^i\cup \colminus)$, $\pbody{\r_{i+1}}\subseteq
V^i$ and 
\[E^{r_{i+1}}= \bigcup_{p\in \pbody{\r_{i+1}}} \{(\rp,\r_{i+1})\mid \rp\in V^i,
\head{\rp}=p\}.\]
Define $(V,E)=\left(\bigcup_{i < \omega} V^i,\bigcup_{i<\omega}
  E^i\right)$. 
Clearly, we have $\colplus \subseteq V$, $\colminus \cap V=\emptyset$ by
construction of $V^i$ for all $i<\omega$.
Furthermore, $E$ contains no cycles because $E'$ contains further
edges are only from $V^i$ to $V^{i+1}$ for $i < \omega$ and we have
$\pbody{\r}\subseteq \{\head{\rp} \mid (\rp,\r)\in E\}$ for all $\r\in V$. 
Thus, $(V,E)$ is a support graph of $(\bg{},\col)$.
Furthermore, this support graph is maximal wrt vertices by the construction
of $V$.

\end{proof}
%%% Local Variables: 
%%% mode: latex
%%% TeX-master: t
%%% End: 


==> Proofs/LongVersion/thm_nlp_properties.tex <==

%---------------------------------------------------------------
\begin{proof}{thm:nlp:properties}
Let $\bg{}$ be the \RDGraph\ of logic program $\Pi$,
$\col$ be a partial 
coloring 
of $\bg{}$ and $X \in \AS{\Pi}{\col}$.
By definition of $X$, we have $\colplus\subseteq  \GR{\Pi}{X}$ and by
Theorem~\ref{thm:X:headcolplus} 
$\head{\colplus}\subseteq X$.
  
%
\paragraph{Show condition 1:}
%
Let $\r\in S(\bg{},\col)$.
%
Then, for all $p \in \pbody{\r}$ there exists an $\rp \in \Pi$ such that
$(\rp,\r)\in \bgezero$, $p=\head{\rp}$ and $\rp\in\colplus$.
%
From $\head{\colplus}\subseteq X$, we can reconclude that for each $p \in
\pbody{\r}$, we have $p \in X$, and thus $\pbody{\r}\subseteq X$.
%
\paragraph{Show condition 2:}
% 
Let  $\r \in \overline{S}(\bg{},\col)$. 
% 
Then for all rules $\rp \in \Pi$ such that $\head{\rp}=p$ we have that
$\rp\in\colminus$ for some $p \in \pbody{\r}$.
%
By Theorem~\ref{cor:X:headcolplus}, we have $p \not \in X$ and thus 
$\pbody{\r}\not\subseteq X$. 
%
\paragraph{Show condition 3:}
%
Let $\r\in B(\bg{},\col)$.
Then, \r\ is blocked by some $\rp\in \colplus$ and $q=\head{\rp}\in
\nbody{\r}$ by 
definition of the 
\RDGraph. 
Because $\head{\colplus}\subseteq X$, we have $q \in X$ and thus
$\nbody{\r} \cap X \not= \emptyset$.   
%
\paragraph{Show condition 4:}
% 
Let $\r \in \overline{B}(\bg{},\col)$, then for all $\rp\in \Pi$ such that
$(\rp,\r)\in 
\bgeone$,  we have $\rp \in\colminus$.
%  
By Theorem~\ref{cor:X:headcolplus} and by the definition of the \RDGraph, 
for all $q\in \nbody{\r}$ we have that 
$q\not\in X$ and thus $\nbody{\r} \cap X = \emptyset$.

\end{proof}
%----------------------------------------------------------------

%%% Local Variables: 
%%% mode: latex
%%% TeX-master: t
%%% End: 


==> Proofs/ShortVersion/prop_AS_maxSG.tex <==
\begin{proof}{prop:AS:maxSG}
  Let $\bg{}$ be the \RDGraph{} for logic program $\Pi$, 
  $\col$ be a total coloring of $\bg{}$ 
  and  
  $X$ be a set of atoms such that $\GR{\Pi}{X}=\colplus$ and
  $X=\head{\colplus}$. 
For this proof we use Theorem~\ref{thm:acoloring:sets} for a characterisation
  of an answer set.

\paragraph{"$\Rightarrow$"}
By Theorem~\ref{thm:acoloring:sets} there exists a  support graph
of $(\bg{},\col)$.
This is $(\colplus,E)$ for some $E\subseteq (\Pi\times\Pi)$ by definition.
But $(\colplus,E)$ is also a support graph of
$\bg{}|_{\overline{B}(\bg{},\col)}$ 
by $\overline{B}(\bg{},C)\cap \GR{\Pi}{X}=\emptyset$
(Corollary~\ref{cor:nlp:properties}). 
%% because for all $\r\in B(\bg{},\col)$ we
%% have $\r\not\in\colplus=\GR{\Pi}{X}$ by Corollary~\ref{cor:nlp:properties}.

% Because for all $\r\in \bg{}\setminus
% \bg{}|_{\overline{B}(\bg{},\col)}$ we have that \r\ is \ablocked\ in
% $(\bg{},\col)$, we have
% $\r\not\in \GR{\Pi}{X}$ and $\r\not\in \colplus$.
% Therefore there exists a maximal support graph of
% $\bg{}|_{\overline{B}(\bg{},\col)}$.
% This must be $(\colplus,E)$ for some $E\subseteq (\Pi\times\Pi)$ because we
% have a total coloring $\col$.

\paragraph{"$\Leftarrow$"}
With Theorem~\ref{thm:acoloring:sets} it is enough to show that $\colplus =
S(\bg{},\col)\cap\overline{B}(\bg{},\col)$.
The existence of a support graph of $(\bg{},\col)$ is ensured because
\col\ is total and we have a  support graph of
$\bg{}|_{\overline{B}(\bg{},\col)}$ because for
all $\r\in \bg{}\setminus \bg{}|_{\overline{B}(\bg{},\col)}$ we have $r\in
B(\bg{},\col)$ and $\r\in \colminus$. 

Clearly, $\colplus \subseteq
S(\bg{},\col)\cap\overline{B}(\bg{},\col)$ because for all $\r\in
\colplus$ we have that $r\in S(\bg{},\col)$ because \r\ is in the
support graph and $r\in \overline{B}(\bg{},\col)$ because \r\
is a vertex of the 
graph $\bg{}|_{\overline{B}(\bg{},\col)}$.

Assume, $\colplus \not\supseteq
S(\bg{},\col)\cap\overline{B}(\bg{},\col)$.
Then, there exists an $r\in
S(\bg{},\col)\cap\overline{B}(\bg{},\col)$ such that $r\in
\colminus=\Pi\setminus \GR{\Pi}{X}$.
Then, we have either $\pbody{r}\not\subseteq X$ or $\nbody{r}\cap
X\not=\emptyset$. 
If $\nbody{r}\cap X\not=\emptyset$ then $\nbody{r}\cap \head{\colplus}
\not=\emptyset$. 
Thus, $r\in B(\bg{},C)$, but this is a contradiction to  $r\in
\overline{B}(\bg{},C)$.
If $\pbody{r}\not\subseteq X$ then $\pbody{r}\not\subseteq \head{\colplus}$ by
$X=\head{\colplus}$.
Thus, $r\not\in S(\bg{},C)$ which is also a contradiction.
Thus, $r\in \colplus$.

%%  because for all $\r\in
%% S(\bg{},\col)\cap\overline{B}(\bg{},\col) $ we have with
%% Corollary~\ref{cor:nlp:properties} that $\pbody{\r}\subseteq X$ and
%% $\nbody{\r}\cap X=\emptyset$.
%% Thus, $\r\in \GR{\Pi}{X}=\colplus$.



\end{proof}
%%% Local Variables: 
%%% mode: latex
%%% TeX-master: t
%%% End: 


==> Proofs/ShortVersion/prop_SG_existence.tex <==
\begin{proof}{prop:SG:existence}
  Let \bg{} be the \RDGraph{} of logic program $\Pi$.
  Let
  $(V,E),(V',E')$ be  support graphs of $\bg{}$ for some $E,E'\subseteq
  (\Pi\times \Pi)$ such that $V \not=V'$.
  Then, we show that there exists a support graph $(V^\ast,E^\ast)$ of $\bg{}$
  for some $E^\ast\subseteq  (\Pi\times \Pi)$ such that $V\subseteq V^\ast$
  and $V'\subseteq V^\ast$.
  By $\Pi$ is finite and by finiteness of the number of all support graphs, we
  can conclude that there exists a maximal support graph of \bg{}.

Assume, there exists a maximal support graph $(V',E')$ of $\bg{}$ for some
$E'\subseteq (\Pi\times \Pi)$ such that $V' \not= V$.

Let $\langle r_i\rangle_{0 \leq i \leq n}$ be an enumeration of $V$ such that
$\pbody{r_i}\subseteq\{\head{r_j}\mid j < i\}$ and  
 $\langle r'_i\rangle_{0 \leq i \leq m}$ be an enumeration of $V'$ such that
$\pbody{r'_i}\subseteq\{\head{r'_j}\mid j < i\}$.

Now, we want to construct an enumeration $\langle s_i\rangle_{0 \leq i \leq
  k}$ such that 
\begin{enumerate}
\item $V^\ast= \{s_i \mid 0\leq i \leq k\}$,
\item $V \subseteq V^\ast$,
\item $V' \subseteq V^\ast$ and
\item $(V^\ast,E^\ast)$ is a support graph of $\bg{}$ for some
  $E^\ast\subseteq (\Pi\times\Pi)$.
\end{enumerate}

Define inductively $\langle s_i \rangle_{0 \leq i \leq k}$ by
$s_0=r_0$ and 
\[
s_i = \left\{   
  \begin{array}{ll}
    r_j & \text{ for } j \leq n \text{ such that } 
          \pbody{r_j}\subseteq\{\head{s_l}\mid l < i\}
          \text{ or }\\
    r'_j & \text{ for } j \leq m \text{ such that } 
          \pbody{r'_j}\subseteq\{\head{s_l}\mid l < i\}\\
    r    & r\in\Pi, \pbody{r}\subseteq \{\head{s_l}\mid l < i\}
  \end{array}
      \right.
\]
for $0 < i \leq k$ where $k = 1+n + m - |V \cap V'|$.

Define $V^\ast= \{s_i \mid 0\leq i \leq k\}$.
By construction of $V^\ast$ we have $V \subseteq V^\ast$ and $V'\subseteq
V^\ast$. 

Define $E^\ast = \bigcup_{0 \leq i \leq k} E^i$ where
\[
E^i= \bigcup_{p \in \pbody{s_i}} \{(\rp,s_i)\mid \head{\rp}=p,
\rp\in\{s_0,\ldots,s_{i-1}\}\}. 
\]
Clearly, $(V^\ast,E^\ast)$ is a acyclic \subgraph{0}\ by construction.
Furthermore, $(V^\ast,E^\ast)$ is a support graph of $\bg{}$.



% Let $\bg{}$ be the \RDGraph{} of logic program $\Pi$.

% Assume that we have two maximal support graphs $(V_1,E_1)$ and $(V_2,E_2)$
% of $\bg{}$ such that $V_1 \not\subseteq V_2$ and $V_2 \not\subseteq V_1$.

% Now we show that $(V_1 \cup V_2,E)$ is a maximal support graph for some
% $E\subseteq (\Pi \times \Pi)$.
% This is then a contradiction to the assumption and thus there exists only one
% maximal (wrt. set of vertices) support graph of $\bg{}$.

% We can choose $E=E_1 \cup E_2$.
% Then, $E_1$ and $E_2$ can be chosen in this way, that $E$ is acyclic. 
% If this is not the case, then $E_1$ or $E_2$ must contain cycles because of
% the definition of a support graph.
% But that is a contradiction to the assumption that $(V_i,E_i)$ are support
% graphs for $i\in \{1,2\}$.
% \comment{K: i know that it is schwammig}

% Clearly, we have for all $r \in V_1 \cup V_2$ that $\pbody{\r}\subseteq
% \{\head{\rp}\mid (\rp,\r)\in E_1 \cup E_2\}$.
% So, $(V_1 \cup V_2,E_1\cup E_2)$ is a support graph of $\bg{}$.



\end{proof}
%%% Local Variables: 
%%% mode: latex
%%% TeX-master: t
%%% End: 


==> Proofs/ShortVersion/thm_acol_acolorings_ver1.tex <==
\begin{proof}{thm:acol:acolorings:ver1}

To show this corollary we show the equivalence to the conditions given in
Theorem~\ref{thm:acol:acolorings:ver2}.
Clearly, a support graph of $(\bg{},C)$ is actually $(\colplus,E)$ for some
$E\subseteq \Pi\times\Pi$ by Definition~\ref{def:acol:maxgrounded}. 
%
Furthermore, conditions~2 and~3 of
Corollary~\ref{thm:acol:acolorings:ver1} are equivalent to 
conditions~1 and~2 in Definition~\ref{def:acol:onedsg} of a  blockage graph.

%% the existence of a
%% blockage graph:
%% \[(S,\bgeone|_S) \text{ is a blockage graph of }$(\bg{},C)$\text{ where }
%%   S=S(\bg{},\col)\]
%% iff
%% \begin{description}
%%   \item[C~1:] for all $\r\in (\colminus\cap{S}(\bg{},\col))$ there exists an
%%     $\rp \in \colplus$ such that $(\rp,\r)\in \bgeone$; 
%%   \item[C~2:] there are no $\r,\rp \in \colplus$
%%     such that $(\r,\rp)\in \bgeone$.
%% \end{description}

%% We will remark that all rules $\r \in \Pi\setminus S(\bg{},\col)$ are colored
%% with $\cminus$.
%% Otherwise $(\colplus,E)$ is no support graph of $(\bg{},\col)$, because an
%% \anotgrounded\ rule could not be in a support graph.
%% Condition C~2 corresponds directly to condition~1 of a blockage graph in
%% Definition~\ref{def:acol:onedsg}. 
%% Even under regard that $\colplus\subseteq S(\bg{},\col)$ because
%% $(\colplus,E)$ is a support graph of $(\bg{},\col)$.

%% Condition C~1 corresponds directly to condition~1 of a blockage graph in
%% Definition~\ref{def:acol:onedsg} by $\colplus \subseteq S(\bg{},\col)$ and
%% thus $\colplus \cap S(\bg{},\col)=\colplus$. 


\end{proof}
%%% Local Variables: 
%%% mode: latex
%%% TeX-master: t
%%% End: 


==> Proofs/ShortVersion/thm_acol_acolorings_ver2.tex <==
\begin{proof}{thm:acol:acolorings:ver2}
  Let  $\bg{}=(\bgv,\bgezero,\bgeone)$ be the \RDGraph{} of a logic program
  $\Pi$. 
  
  Furthermore, 
  let $\col$ be a total coloring of \bg{}
  and
  $X$ be a set of atoms such that
  \(
  \GR{\Pi}{X}=\colplus
  \) $X=\head{\colplus}$.

\paragraph{``$\Rightarrow$''}
Let $X$ be an answer set, then by Theorem~\ref{thm:acoloring:sets} there
exists some support graph of $(\bg{},\col)$.
Hence, it remains to show, that $(S,\bgeone|_S)$ is a blockage graph of
$(\bg{},C)$ where  $S=S(\bg{},\col)$.

For all $\r\in \colplus$ we have $r\in\overline{B}(\bg{},\col)$ by
Theorem~\ref{thm:acoloring:sets}.
Thus, condition~1 for a blockage graph in Definition~\ref{def:acol:onedsg}
holds. 

Let $\r\in S\cap \colminus$. 
We have $\pbody{\r}\subseteq X$ and $\r\not\in
\GR{\Pi}{X}$ by Corollary~\ref{cor:nlp:properties} and the definition of
$\GR{\Pi}{X}$.  
Thus, $\nbody{\r}\cap X \not=\emptyset$ by the definition of the \RDGraph\ and
\r\ is blocked by some $\rp\in 
\colplus $ (Corollary~\ref{cor:nlp:properties}).
Hence, condition~2 from Definition~\ref{def:acol:onedsg} holds.
Thus, $(S,\bgeone|_S)$ is a blockage graph of
$(\bg{},C)$.

\paragraph{``$\Leftarrow$''}
It remains to show that $\colplus =
S(\bg{},\col)\cap\overline{B}(\bg{},\col)$ by Theorem~\ref{thm:acoloring:sets}. 
\subparagraph{Show "$\subseteq$":}
Let $\r\in \colplus$. Then $\r\in S(\bg{},\col)$ by $(\colplus,E)$ is
a support graph of $(\bg{},\col)$ for some $E\subseteq (\Pi\times\Pi)$ and by
Definition~\ref{def:acol:maxgrounded}.
Assume, $\r\in B(\bg{},\col)$ then there exists an $\rp\in \colplus$ such that
$(\rp,\r)\in E_1$.
But this is a contradiction to condition~1 in
Definition~\ref{def:acol:onedsg} of a blockage graph.
Thus, $\r\in \overline{B}(\bg{},\col)$.
\subparagraph{Show "$\supseteq$":}
Let $\r\in S(\bg{},\col)\cap\overline{B}(\bg{},\col)$.
We have to show that $\r\in \colplus$.
Assume $\r\in \colminus$.
Then, by condition~2 in Definition~\ref{def:acol:onedsg} of a blockage graph
there exists an $\rp\in  \colplus$ such that $\r$ is blocked by $\rp$.
That's a contradiction and thus $\r\in \colplus$.
% %
% Let $X$ be a set of atoms and $\col$ be a total coloring with the given
% properties.  
% In section~\ref{sec:original} we have that $X$ is an answer set iff $\col$ is
% an \acolorings.
% %
% For the definition of an \acoloring\ we use definition~\ref{def:acoloring}.
% %
% That is, $\col$ is an \acoloring\ if
% \begin{enumerate}
% \item $\r\in \colplus$ if \r\ is grounded and not blocked;
% \item $\r\in \colminus$ if \r\ is not grounded or \r\ is blocked.
% \end{enumerate}
% %
% The definitions of \r\ is blocked, not blocked and not grounded coincide with
% \r\ is \ablocked, \anotblocked\ and \anotgrounded\ in $(\bg{},\col)$ in
% definition~\ref{def:acol:vertexproperties}.
% %
% Now, we will prove the theorem through $\col$ is an \acoloring\ iff 
%   \begin{enumerate}
%   \item there is some \groundedZeroDAG{} of $(\bg{},\col)$ 
%     and
%   \item  $(S,\bgeone|_S)$ is a blockage graph of $(\bg{},C)$ where
%   $S=S(\bg{},\col)$. 
%   \end{enumerate}

% \paragraph{``$\rightarrow$''}
% The existence of a support graph of $(\bg{},\col)$ is ensured through
% theorem~\ref{thm:supportgraph}.
% %
% We have to show that $(S,\bgeone|_S)$ is a blockage graph of $(\bg{},C)$ for
%   $S=S(\bg{},\col)$.
% %
% Let $\r\in S$.
% %
% Then the following cases must be fulfilled:
% \begin{description}
% \item[case 1:] $\r\in \colminus$ if there exists an $(\rp,\r)\in \bgeone$ such
%   that $\rp\in  \colplus$ 
% \item[case 2:] $\r\in\colplus$ if there exists no  $(\rp,\r)\in \bgeone$ such
%   that $\rp\in  \colplus$ 
% \end{description}
% %
% We will mention that we have for all rules $\r \in \Pi\setminus S$ that $\r\in
% \colminus$. 
% %
% Because $\r\in\Pi\setminus S$ means \r\ is \anotgrounded\ we have through
% corollary~\ref{cor:nlp:properties} that $\pbody{\r}\not\subseteq X$ and so
% $\r\not\in \GR{\Pi}{X}$.
% %
% For this, we can restrict $(\rp,\r)\in \bgeone$ to $(\rp,\r)\in \bgeone|_S$.

% Case~1 and case~2 are fulfilled because $\col$ is an \acoloring.
% A rule \r\ is blocked if there exists an $\rp \in \colplus$ such that
% $(\rp,\r)\in E_1$.
% Thus \r\ is colored with $\cminus$ (case~1).
% A rule \r\ is unblocked if for all \rp\ such that $(\rp,\r)\in E_1$ we have
% $\rp \in \colminus$.
% Furthermore \r\ is grounded, because of the support graph there exists a
% $\cplus$ colored grounded-0-graph, and thus colored with $\cminus$.
% % {\bf case 1:}
% % %
% % If $\rp \in \colplus$ and $(\rp,\r)\in \bgeone|_S$ then must \r\ be colored
% % with $\cminus$ because of condition 1 in definition~\ref{def:acol:onedsg} of a
% % blockage graph. 
% % %

% % {\bf case 2:}
% % %
% % Assume that $\r\in \colminus$.
% % %
% % But then, there must exists an $(\rp,\r)\in \bgeone|_S$ such that $\rp\in
% % \colplus$ because of condition 2 in definition~\ref{def:acol:onedsg}.
% % %
% % But that's a contradiction and $\r\in \colplus$.


% \paragraph{``$\leftarrow$''}
% %
% Let $(\bg{},\col)$ be a colored \RDGraph\ with the demanded properties.
% %
% We have to show that $\col$ is an \acoloring.
% %
% Let $\r\in\colplus$.
% %
% We have to show that \r\ is grounded and \anotblocked.
% %
% Because there exists a support graph $(V,E)$ of $(\bg{},\col)$ and $\colplus
% \subseteq V$ we have that \r\ is a vertex in the support graph.
% %
% Through the properties of a support graph, we have also that there exists a
% grounded 0-graph for \r\ such that all vertices of it are colored with
% $\colplus$. 
% %
% Thus, \r\ is grounded.
% %
% So \r\ is \agrounded\ and $\r\in S(\bg{},\col)$.
% %
% Through condition~1 in definition~\ref{def:acol:onedsg} of a blockage graph,
% we have that 
% there is no $(\rp,\r)\in \bgeone$ such that $\rp\in \colplus$.
% Thus, \r\ is \anotblocked.
% %
% Furthermore, all $\r\in \Pi \setminus S(\bg{},\col)$ are colored with
% $\cminus$.
% \comment{K: more rumlabern?}
% So, the restriction of all edges between \agrounded\ rules in a blockage graph
% is not really a
% restriction for deciding if a rule is \ablocked\ or not.

% Now, let $\r\in \colminus$.
% %
% We have to show that \r\ is \anotgrounded\ or \ablocked.
% %
% Assume $\r\in S(\bg{},\col)$.
% %
% Through condition 2 of definition~\ref{def:acol:onedsg} there must exist an
% $(\rp,\r)\in \bgeone|_S$ such that $\rp\in \colplus$.
% %
% Thus, \r\ is blocked.
% %
% Assume $\r\not\in S(\bg{},\col)$.
% %
% Then \r\ is  \anotgrounded\ and we have that \r\ is either \ablocked\ or
% \anotgrounded\ for $\r\in \colminus$.
% \comment{K: alle Faelle erwischt?}

\end{proof}
%%% Local Variables: 
%%% mode: latex
%%% TeX-master: t
%%% End: 


==> Proofs/ShortVersion/thm_acoloring_sets.tex <==
\begin{proof}{thm:acoloring:sets}
  Let $\bg{}$ be the \RDGraph{} of logic program  $\Pi$.
  Furthermore, 
  let $\col$ be a total coloring of \bg{} 
  and
  $X$ be a set of atoms such that $\GR{\Pi}{X}=\colplus$ and
  $X=\head{\colplus}$. 


\paragraph{"$1 \Rightarrow 2$":}
By Theorem~\ref{thm:max:supported:graph:existence} and $\{X\}=\AS{\Pi}{C}$
there exists a 
support graph of $(\bg{},\col)$.
For this reason, it remains to show that $\colplus =
S(\bg{},\col)\cap\overline{B}(\bg{},\col)$.
But this holds by Theorem~\ref{thm:col:gr} and $\colplus=\GR{\Pi}{X}$.
%% \subparagraph{Show "$\subseteq$":}
%% For all $\r\in \GR{\Pi}{X}=\colplus$ we have $\pbody{\r}\subseteq X$ and
%% $\nbody{\r}\cap X =\emptyset$ by the definition of $\GR{\Pi}{X}$.
%% Therefore by Corollary~\ref{cor:nlp:properties} we have 
%% $\colplus \subseteq S(\bg{},\col)\cap\overline{B}(\bg{},\col)$.
%% \subparagraph{Show "$\supseteq$":}
%% Let $\r \in S(\bg{},\col)\cap\overline{B}(\bg{},\col)$ then by
%% Corollary~\ref{cor:nlp:properties} and by definition of $\GR{\Pi}{X}$ we have
%% that $\r\in \GR{\Pi}{X}=\colplus$. 
%% Therefore, $ S(\bg{},\col)\cap\overline{B}(\bg{},\col)\subseteq \colplus$.

\paragraph{"$2 \Rightarrow 1$":}
%% We have to show that $X$ is an answer set, that is $\Cn{\Pi^X}=X$.
%% With Theorem~\ref{thm:as:consGR} it is enough to show that
%% $X=\Cn{(\GR{\Pi}{X})^\emptyset}$. 
Because $\col$ is a total coloring we have $\GR{\Pi}{X}=\colplus=\Pi\setminus
\colminus$.
Because we have a maximal support graph $(V,E)$ of $(\bg{},\col)$ for some
$E\subseteq (\Pi \times \Pi)$ we can conclude
$\head{V}=\Cn{(\Pi\setminus\colminus)^\emptyset}$ by
Theorem~\ref{thm:max:supported:graph:C}.  
Furthermore, by Definition~\ref{def:acol:maxgrounded} we must have $V=\colplus$ because $\col$ is a total coloring.
Thus,
$X=\head{\colplus}=\Cn{(\Pi\setminus\colminus)^\emptyset}=\Cn{(\GR{\Pi}{X})^\emptyset}$  
and therefore $X$ is an answer set by Theorem~\ref{thm:as:consGR}.

% For this proof we use theorem~\ref{thm_coloring} and the
% definition~\ref{def:acoloring} of an \acoloring.

% Clearly, we have that \r\ is supported in $(\bg{},\col)$ if \r\ is grounded
% wrt \bg{}. 

% \paragraph{"$\Rightarrow$":}
% It is easy to see that we have $\colplus =
% S(\bg{},\col)\cap\overline{B}(\bg{},\col)$.
% It remains to show, that there exists a maximal support graph.
% But through theorem~\ref{thm:supportgraph} the existence is ensured.

% \paragraph{"$\Leftarrow$":}
% Through the existence of the support graph we ensure that there exists a
% grounded-0-graph $(V,E)$ for every $\r\in \colplus$ such that $V \subseteq
% \colplus$.
% The other properties follow immediately and $\col$ is an \acoloring.

\paragraph{"$2 \Leftrightarrow 3$":}
The equivalence  holds by $\col$ is a total coloring.
\end{proof}
%%% Local Variables: 
%%% mode: latex
%%% TeX-master: t
%%% End: 


==> Proofs/ShortVersion/thm_max_supported_graph_C.tex <==
\begin{proof}{thm:max:supported:graph:C}
  Let $\bg{}$ be the \RDGraph{} of logic program $\Pi$,
  $C$ be a partial coloring
  and 
  $(V,E)$ be a maximal \groundedZeroDAG{} of $(\bg{},\col)$.


For brevity, we sometimes denote $\Pi'$ as the positive logic program
$\reduct{(\Pi\setminus\colminus)}{\emptyset}$.

We have the equation
\[
\Cn{\Pi'}=\bigcup_{i \geq 0} \Ti{i}{\Pi'}{\emptyset}.
\]
Thus, it is enough to show that 
\[
\bigcup_{i \geq 0} \Ti{i}{\Pi'}{\emptyset}=\head{V}.
\]

This could be proven by induction over $i$ using Equation~\ref{eq:T} and the
maximality of $V$.
%
%% Clearly, we have $\Ti{0}{\Pi'}{\emptyset}=\emptyset \subseteq \head{V}$ and 
%% \(  \Ti{1}{\Pi'}{\emptyset}  = 
%%      \{\head{\r} \mid \r \in (\Pi\setminus \colminus)^\emptyset,
%%   \pbody{\r}=\emptyset\}
%% \).
%% Therefore $\Ti{1}{\Pi'}{\emptyset}\subseteq \head{V}$ by
%% maximality of $V$.
%% Assume, that we have $\Ti{i}{\Pi'}{\emptyset}\subseteq \head{V}$.
%% Then,
%% \begin{eqnarray*}
%%   \Ti{i+1}{\Pi'}{\emptyset} &  = & \{\head{\r}\mid \r\in \Pi',
%%   \body{\r}\subseteq 
%%   \Ti{i}{\Pi'}{\emptyset}\}\\
%%   & \subseteq & \{\head{\r} \mid \r \in \Pi', \body{\r}\subseteq \head{V}\}\\
%%   & \subseteq & \head{V} \text{ (by maximality of $V$) }
%% \end{eqnarray*}
%% Thus, $\Cn{(\Pi\setminus \colminus)^\emptyset}\subseteq \head{V}$.
%
% Clearly, we have $\Ti{0}{\Pi'}{\emptyset}=\emptyset \subseteq \head{V}$.
% For $i=1$ we have $\Ti{1}{\Pi'}{\emptyset}=\{\head{\r}\mid \head{\r}\LPif\;
% \in 
% \Pi'\} \subseteq \head{V}$ because $\r\in \colplus \subseteq V$ for all rules
% $\head{\r}\LPif\; \in \Pi'$.
% Assume, that we have $\Ti{i}{\Pi'}{\emptyset}\subseteq \head{V}$ for some
% $i\geq 0$.
% Then,
%
% $\begin{array}{ll}
% \Ti{i+1}{\Pi'}{\emptyset}& = \Ti{}{\Pi'}{\Ti{i}{\Pi'}{\emptyset}}\\
% & = \{\head{\r} \mid \r\in \Pi', \body{\r}\subseteq \Ti{i}{\Pi'}{\emptyset}
% \}\\ 
% & = \{\head{\r} \mid \r\in \Pi', \body{\r}\subseteq \head{V}\}\\
% & \subseteq \head{V}.
% \end{array}$
% The last ``$\subseteq$'' follows because \r\ must be a element of the maximal
% support graph.
%
%% \paragraph{Show "$\supseteq$"}
%% There exists an
%% enumeration $\langle r_i 
%% \rangle_{0\leq i \leq n}$ of $V$ such that $\pbody{r_i}\subseteq
%% \head{\{r_j\mid j<i\}}$ for all $0\leq i\leq n$ by the definition of a support
%% graph.
%% We have to show, that  $\head{r_i}\in \bigcup_{j < \omega}
%% \Ti{j}{\Pi'}{\emptyset}$ for all $0\leq i \leq n$.
%
%% By $\pbody{r_0}=\emptyset$ we have $\head{r_0}\in \bigcup_{j < \omega}
%% \Ti{j}{\Pi'}{\emptyset}$.
%% Assume that $\head{r_i}\in\bigcup_{j < \omega}\Ti{j}{\Pi'}{\emptyset} $ for all
%% $i < k < n$.
%% We have to show that $\head{r_k}\in\bigcup_{j<\omega}\Ti{j}{\Pi'}{\emptyset}$.
%% We have $\pbody{r_k}\subseteq \head{\{r_i\mid i < k\}}\subseteq \bigcup_{j<
%%   \omega }\Ti{j}{\Pi'}{\emptyset}$.
%% In detail, there exists some $l<\omega$ 
%% \comment{or $l<k$?}
%% such that 
%% $\pbody{r_k}\subseteq \bigcup_{0\leq j \leq l}\Ti{j}{\Pi'}{\emptyset}$.
%% By Equation~\ref{eq:T} we have  
%% $\head{r_k}\in\bigcup_{0\leq j \leq l+1}\Ti{j}{\Pi'}{\emptyset}$ and thus
%% $\head{V}\subseteq \bigcup_{j < \omega}\Ti{j}{\Pi'}{\emptyset}$.
%
%
% Clearly, we have $\head{\colplus}=\Ti{1}{\Pi'}{\emptyset}$.
% Assume, that we have $\head{V'}\subseteq 
% \Ti{n}{\Pi'}{\emptyset} $ for some not maximal support graph $V'$ and $n \geq
% 0$. 
%
% Let be $\r \in \Pi'$ such that $\r\in V\setminus V'$ and $\body{\r}\subseteq
% \head{V'}$.
% Such an \r\ must exist because $V'$ is not maximal.
% Then, we have $\body{\r}\subseteq \Ti{n}{\Pi'}{\emptyset} $.
% So, $\head{\r}\subseteq \Ti{}{\Pi'}{\Ti{n}{\Pi'}{\emptyset}} \subseteq
% \bigcup_{i \geq 0} \Ti{i}{\Pi'}{\emptyset}$.
%
% This induction works, because we have only one maximal support graph wrt the
% vertices, see~\ref{thm:max:supported:graph:existence}. 
\end{proof}
%%% Local Variables: 
%%% mode: latex
%%% TeX-master: t
%%% End: 


==> Proofs/ShortVersion/thm_red.tex <==
\begin{proof}{thm:red}
%
Let \bg{}  be the \RDGraph\ of logic program $\Pi$, $\col$ be a total coloring 
of \bg{} and $X$ be a set of atoms such that $\GR{\Pi}{X}=\colplus$.
%
\paragraph{Show "$\Leftarrow$":}
%
If $\r\in \overline{B}(\bg{},\col)$ then 
we have $\nbody{\r}\cap X =\emptyset$ by Corollary~\ref{cor:nlp:properties}.
%
From the definition of $\Pi^X$ we have $\head{\r} \LPif \pbody{\r} \in
\Pi^X$. 
\paragraph{Show "$\Rightarrow $":}
Let $\r\in \Pi$ such that $\head{\r}\LPif \pbody{\r} \in \Pi^X$, then
$\nbody{\r}\cap X=\emptyset$ by definition of $\Pi^X$.
Thus, by Corollary~\ref{cor:nlp:properties} we have  $\r\in
\overline{B}(\bg{},\col)$.  
% \paragraph{Show "$2 \Rightarrow 3$":}
% Let $\r\in \overline{B}(\bg{},\col)$ then we have either $\r\in
% \overline{S}(\bg{},\col)$ or $\r\not\in \overline{S}(\bg{},\col)$, i.e. $\r\in
% S(\bg{},\col)$ because
% \col\ is total.
% If $\r\in \overline{S}(\bg{},\col)$ then we have $\r\in
% \overline{B}(\bg{},\col) \cap \overline{S}(\bg{},\col)$.
% Otherwise, if $\r\in S(\bg{},\col)$ then $\pbody{\r}\subseteq X$ and
% $\nbody{\r}\cap X=\emptyset$ by Corollary~\ref{cor:nlp:properties}.
% Thus, $\r\in \GR{\Pi}{X}=\colplus$ and $\head{\r}\LPif\; \in \Pi^\col$ by
% definition of $\Pi^\col$.
% \paragraph{Show "$3 \Rightarrow 2$":}
% If we have $\r\in  \overline{B}(\bg{},\col) \cap \overline{S}(\bg{},\col)$
% then clearly $\r\in \overline{B}(\bg{},\col)$.
% Otherwise, if $\head{\r}\LPif\; \in \Pi^\col$ then by definition of $\Pi^C$ we
% have $\r\in\colplus$.
% Thus, we have $\r\in \GR{\Pi}{X}=\colplus$ and $\nbody{\r}\cap X=\emptyset$ by
% definition of $\GR{\Pi}{X}$.
% Thus, \r\ is unblocked in $(\bg{},\col)$ by Corollary~\ref{cor:nlp:properties}.
\end{proof}
%%% Local Variables: 
%%% mode: latex
%%% TeX-master: t
%%% End: 


==> Proofs/ShortVersion/thm_supportgraph.tex <==
\begin{proof}{thm:supportgraph}
This follows from $\AS{\Pi}{C}\not=\emptyset$, $C$ is a total coloring,
Theorem~\ref{thm:max:supported:graph:existence} and
Definition~\ref{def:acol:maxgrounded}.  
%% Let \bg{} be the \RDGraph\ of logic program $\Pi$ and $X$ an answer set of
%% $\Pi$.
%% %
%% Furthermore, let $\col$ be a total coloring such that $\colplus=\GR{\Pi}{X}$
%% and $\colminus=\Pi \setminus \GR{\Pi}{X}$.
%% %
%% By $\AS{\Pi}{C}\not=\emptyset$ and
%% Theorem~\ref{thm:max:supported:graph:existence}, there exists a support graph
%% of $(\bg{},C)$.
%% This must be $(\colplus,E)$  for some $E\subseteq \Pi\times\Pi$.
%% Because $\col$ is total, a support graph of $\bg{}|_\col$ is a support graph
%% of $\bg{}$.
%% We have to show, that $(\colplus,E)$ is a  support graph of
%% $\bg{}|_\col=\bg{}$ for some $E \subseteq 
%% (\Pi\times \Pi)$. 
%% By Theorem~\ref{thm:max:supported:graph:existence}, $(\colplus,E)$ is then a
%% maximal support graph of $(\bg{},\col)$ because $\col$ is a total coloring. 
%% Analogous to Theorem~\ref{thm:max:supported:graph:existence} we can
%% construct a support graph $(\colplus,E)$ for some $E \subseteq
%% (\Pi\times \Pi)$ starting from an enumeration  of $\GR{\Pi}{X}=\colplus$. 
%% \comment{reproof it!}
% Through theorem~\ref{thm:gr:grounded} there exists an enumeration $\langle r_i
% \rangle_{i \in I}$ of
% $\GR{\Pi}{X}$ such that for all $i \in I$ we have $\pbody{r_i} \subseteq
% \head{\{r_j \mid j <   i\}}$.
% This property gives us directly the existence of an $E\subseteq (\Pi\times
% \Pi)$ such that  $(\colplus,E)$ is a support graph.
\end{proof}
%%% Local Variables: 
%%% mode: latex
%%% TeX-master: t
%%% End: 

